ExMap: Leveraging Explainability Heatmaps for Unsupervised Group Robustness to Spurious Correlations

Group robustness strategies aim to mitigate learned biases in deep learning models that arise from spurious correlations present in their training datasets. However, most existing methods rely on the access to the label distribution of the groups, which is time-consuming and expensive to obtain. As a result, unsupervised group robustness strategies are sought. Based on the insight that a trained model's classification strategies can be inferred accurately based on explainability heatmaps, we introduce ExMap, an unsupervised two stage mechanism designed to enhance group robustness in traditional classifiers. ExMap utilizes a clustering module to infer pseudo-labels based on a model's explainability heatmaps, which are then used during training in lieu of actual labels. Our empirical studies validate the efficacy of ExMap - We demonstrate that it bridges the performance gap with its supervised counterparts and outperforms existing partially supervised and unsupervised methods. Additionally, ExMap can be seamlessly integrated with existing group robustness learning strategies. Finally, we demonstrate its potential in tackling the emerging issue of multiple shortcut mitigation\footnote{Code available at \url{https://github.com/rwchakra/exmap}}.

==> ExMap-3/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames, table]{xcolor}
%\usepackage[table]{xcolor}
\usepackage{tabularx}
\usepackage{algorithm}
\usepackage{mathabx}
\usepackage{amsmath}
\DeclareMathOperator{\sign}{sign}
\usepackage{algpseudocode}
\usepackage{pifont}
\usepackage{float}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{adjustbox}
\usepackage{afterpage}
\usepackage{lipsum} % for dummy text
\usepackage{booktabs} % For prettier tables
\usepackage{siunitx}  % For aligning numbers by decimal point
%\usepackage[dvipsnames]{xcolor}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> ExMap-3/sec/0_abstract.tex <==
\begin{abstract}
% \todo{need to update abstract and related work to reflect that there are mutliple unsupervised approaches now.}
Group robustness strategies aim to mitigate learned biases in deep learning models that arise from spurious correlations present in their training datasets. However, most existing methods rely on the access to the label distribution of the groups, which is time-consuming and expensive to obtain. As a result, unsupervised group robustness strategies are sought. Based on the insight that a trained model's classification strategies can be inferred accurately based on explainability heatmaps, we introduce ExMap, an unsupervised two stage mechanism designed to enhance group robustness in traditional classifiers. ExMap utilizes a clustering module to infer pseudo-labels based on a model's explainability heatmaps, which are then used during training in lieu of actual labels. Our empirical studies validate the efficacy of ExMap - We demonstrate that it bridges the performance gap with its supervised counterparts and outperforms existing partially supervised and unsupervised methods. Additionally, ExMap can be seamlessly integrated with existing group robustness learning strategies. Finally, we demonstrate its potential in tackling the emerging issue of multiple shortcut mitigation\footnote{Code available at \url{https://github.com/rwchakra/exmap}}.
\end{abstract}

==> ExMap-3/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{ExMap/images/exmap_highlevel_new.pdf}
%     %\vspace{-1cm}
%     \caption{A broad outline of ExMap: While other methods require the access to group labels as inputs to the group robustness strategy S, our method generates pseudo-labels for the same. We show that such pseudo-labels improve the worst group accuracy on different datasets.}
%     \label{fig:exmap_highlevel}
% \end{figure}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/exmap_highlevel_new.pdf}\vspace{-2mm}
    %\vspace{-1cm}
    \caption{To improve the original models worst group accuracy, most current approaches rely on supervised group labels (a), which requires extensive annotation processes. Unsupervised approaches have relied on extracting pseudo labels based on the models feature representations (b), where information can be highly entangled. ExMap instead infers group pseudo labels based on explainability heatmaps (c), leading to improved worst group performance.}\vspace{-3mm}
    \label{fig:exmap_highlevel}
\end{figure*}

Deep neural network classifiers trained for classification tasks, have invited increased scrutiny from the research community due to their overreliance on spurious correlations present in the training data \cite{DBLP:journals/corr/abs-2110-04301, brendel2018approximating, Geirhos2018ImageNettrainedCA, Zhang2022, Bahng2019LearningDR}. This is related to the broader aspect of Shortcut Learning \cite{Geirhos2020ShortcutLI}, or the Clever Hans effect \cite{Lapuschkin2019UnmaskingCH}, where a model picks the path of least resistance to predict data, thus relying on shortcut features that are not causally linked to the label. The consequence of this phenomenon is that, although such models may demonstrate impressive mean accuracy on the test data, they may still fail on challenging subsets of the data, i.e. the groups \cite{duchi2023distributionally, duchi2018statistics, Oren2019DistributionallyRL}. As a result, group robustness is a natural objective to be met to mitigate reliance on spurious correlations. Thus, instead of evaluating models based on mean test accuracy, evaluating them on \textit{worst group accuracy} has been the recent paradigm~\cite{Izmailov2022OnFL, Nam2022SpreadSA, Zhou2021ExaminingAC, Lokhande2022TowardsGR}, resulting in the emergence of group robustness techniques. By dividing a dataset into pre-determined groups of spurious correlations, classifiers are then trained to maximize the \textit{worst group accuracy} - As a result, the spurious attribute that the model is most susceptible to is considered the shortcut of interest.

In Figure \ref{fig:exmap_highlevel}, we illustrate the group robustness paradigm. Given a dataset, a robustness strategy takes as input the group labels and retrains a base classifier (such as Expected Risk Minimization, i.e. ERM) to improve the worst group accuracy (G3 in this case). GroupDRO \cite{Sagawa2019DistributionallyRN}  was one of the early influential works that introduced the group robustness paradigm. Further, it demonstrated a strategy that could indeed improve worst group accuracy. One limitation of this approach was the reliance on group labels in the training data, which was replaced with the reliance on group labels in the validation data in successive works \cite{Liu2021JustTT, Kirichenko2022LastLR}. However, while these efforts have made strides in enhancing the accuracy of trained classifiers for underperforming groups, many hinge on the assumption that the underlying groups are known apriori and that the group labels are available, which is often impractical in real-world contexts. An unsupervised approach, as illustrated in Figure \ref{fig:exmap_highlevel}, would ideally estimate pseudo-labels that could be inputs to any robustness strategy, leading to improved worst group robustness. An example of such a fully unsupervised worst group robustness approach is (GEORGE) \cite{Sohoni2020NoSL}. GEORGE clusters the penultimate layer features in a UMAP reduced space, demonstrating impressive results on multiple datasets. In this work, we instead show that clustering \textit{explainability heatmaps} instead, is more beneficial in improving worst group robustness. Intuitively, this stems from the fact that a pixel-attribution based explainability method in input space focuses only on the relevant image features (pixel space) in the task, discarding other entangled features irrelevant for the final prediction.  

In our work, we circumvent the need for a group labeled dataset by introducing ExMap, a novel two stage mechanism: First, we extract explainability heatmaps from a trained (base)
model on the dataset of interest (we use the validation set \textit{without} group labels). Next, we use a clustering module to produce pseudo-labels for the validation data. The resulting pseudo-labels can then be used for any off-the-shelf group robustness learning strategy in use today. ExMap is also flexible in the choice of clustering algorithm. We show that attaching the ExMap mechanism to baseline methods leads to improved performance over the unsupervised counterparts, and  further closes the gap to supervised and partially supervised counterparts. Additionally, we demonstrate that ExMap is also useful in the recent \textit{multiple shortcut} paradigm \cite{Li2022AWD}, where current popular supervised approaches have been shown to struggle. We conclude with an extended analysis on why clustering explainability heatmaps is more beneficial than raw features. In summary, our contributions include:
\begin{itemize}
    \item [1.] ExMap: A simple but efficient unsupervised, strategy agnostic mechanism for group robustness that leverages explainability heatmaps and clustering to generate pseudo-labels for underlying groups. 
    \item [2.] An extended analysis that provides intuition and insight into why clustering explainability heatmaps leads to superior results over other group-robustness baseline methods.
    \item [3.]  Demonstrating the usefulness of ExMap in improving worst group robustness in both the single shortcut and multiple shortcut settings. 
\end{itemize}




% \begin{figure*}[h]
%     \centering
%     \vspace{-5cm}
%     \includegraphics[width=\textwidth]
%     {ExMap/images/exmap.png}
%     \vspace{-3cm}
%     \caption{t-SNE plot of CelebA heatmaps in 2D coloured with ground truth groups. Left: class $y=0$, Right: class $y=1$. It is impossible to recover the ground truth labels here.}
%     \label{fig:tsne_celeba}
% \end{figure*}

==> ExMap-3/sec/2_formatting.tex <==
\section{Related Work}
\label{sec:formatting}

% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% high.
% %
% Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% The \LaTeX\ template takes care of this when used properly.



% %-------------------------------------------------------------------------
% \subsection{Type style and fonts}

% Wherever Times is specified, Times Roman may also be used.
% If neither is available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE.
% Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% Leave two blank lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type.
% This information is to be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT.
% Type main text in 10-point Times, single-spaced.
% Do NOT use double-spacing.
% All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% Make sure your text is fully justified---that is, flush left and flush right.
% Please do not place any additional blank lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% Short captions should be centred.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% FIRST-ORDER HEADINGS.
% (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS.
% (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote{This is what a footnote looks like.
% It often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% Use Times 8-point type, single-spaced.


% %-------------------------------------------------------------------------
% \subsection{Cross-references}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

\paragraph{Single shortcut mitigation with group labels}
The paradigm of taking a frozen base model and proposing a shortcut mitigation strategy to maximise \textit{worst group accuracy} was introduced in Group-DRO (gDRO) \cite{Sagawa2019DistributionallyRN}. However, the requirement of group labels in both training and validation data motivated the proposal of mitigation strategies without training labels. %JTT \cite{Liu2021JustTT} constructs a set of misclassified examples from an ERM model using early stopping, and upweights these samples in the second training phase. The validation labels are used for model selection. DFR \cite{Kirichenko2022LastLR} re-trains the final layer of a base ERM model on a balanced, reweighting dataset, demonstrating improved robustness to the spurious features. LfF \cite{Nam2020LearningFF} first amplifies the biases on the base model, and then uses the misclassified samples to train a debiased model on the error set. Both DFR and Lff require group labels on the validation set, and implicitly capture the concept of retraining representations to specifically capture and discard spurious correlations. BARACK \cite{Sohoni2021BARACKPS} is a partially supervised technique that first uses a small set of group labeled training data to generate pseudo group labels for data with missing annotations. GEORGE \cite{Sohoni2020NoSL} proposes an unsupervised mechanism to generate pseudo-labels for retraining by clustering raw features, and is therefore the closest method to our proposed ExMap. 
This has resulted partially supervised approaches~\cite{Sohoni2021BARACKPS} that only require a small set of group labels as well as in several methods that only require the validation group labels~\cite{Liu2021JustTT,Kirichenko2022LastLR,Nam2020LearningFF}. One such example is DFR\cite{Kirichenko2022LastLR}, which re-trains the final layer of a base ERM model on a balanced, reweighting dataset. Most relevant to our work, GEORGE~\cite{Sohoni2020NoSL} proposes an unsupervised mechanism to generate pseudo-labels for retraining by clustering raw features, and can therefore be considered the closest method to our proposed ExMap.
We show that clustering heatmaps is a more beneficial and intuitive technique for generating pseudo-labels, as attributing the model performance on the input data pixels leads to a more intuitive interpretation of which features are relevant for the task, and which are not. Our method, ExMap, leverages this insight and clusters the heatmaps instead, leading to improved performance over GEORGE and its two variants - GEORGE(gDRO) trained with the Group-DRO strategy, and GEORGE(DFR), trained with the DFR strategy. 
\vspace{-0.25cm}
\paragraph{Other Strategies for Shortcut Mitigation}
There are other extant works that mitigate spurious correlations without adopting the group-label based paradigm directly. MaskTune \cite{Taghanaki2022MaskTuneMS}, for instance, learns a mask over discriminatory features to reduce reliance on spurious correlations. CVar DRO \cite{Lvy2020LargeScaleMF} proposes an efficient robustness strategy using conditional value at risk (CVar). DivDis \cite{Lee2023DiversifyAD}, on the other hand, proposes to train multiple functions on source and target data, identifying the most informative subset of labels in the target data. Discover-and-Cure (DISC) \cite{Wu2023DiscoverAC} discovers spurious concepts using a predefined concept bank, then intervenes on the training data to mitigate the spurious concepts, while ULA \cite{Tsirigotis2023GroupRC} uses a pretrained self-supervised model to train a classifier to detect and mitigate spurious correlations. While these approaches do not directly adopt the group-label, we show that the proposed explainability heatmap-based approach is more efficient in improving the worst-group accuracy.

\paragraph{Multi-Shortcut Mitigation}
The single shortcut setting is a simpler benchmark as the label is spuriously correlated with only a single attribute. However, real world datasets are challenging, and may contain multiple spurious attributes correlated with an object of interest. As a result, when one spurious attribute is known, mitigating the reliance on this attribute may exacerbate the reliance on another. The recently introduced Whac-A-Mole \cite{Li2022AWD} dilemma for multiple shortcuts demonstrates this phenomenon with datasets containing multiple shortcuts (e.g. background and co-occurring object). Single shortcut methods fail to mitigate \textit{both} shortcuts at once, leading to a spurious conservation principle, where if one shortcut is mitigated, the other is exacerbated. The authors introduce Last Layer Ensemble (LLE) to mitigate multiple shortcuts in their datasets, by training a separate classifier for each shortcut. However, LLE's reliance on apriori knowledge of dataset shortcuts is impractical in the real world. We evaluate ExMap in this context and show that it is effective as an unsupervised group robustness approach to the multi-shortcut setting. 
\vspace{-0.25cm}
\paragraph{Heatmap-based Explainability}

The challenge of attributing learned features to the decision making of a model in the image space has a rich history. The techniques explored can be differentiated on a variety of axes. LIME, SHAP,  LRP \cite{Guo2017LIMELI, Lundberg2017AUA, Bach2015OnPE} are early model-agnostic methods, while Grad-CAM and Integrated Gradients\cite{Selvaraju2016GradCAMVE, Sundararajan2017AxiomaticAF} are gradient based attribution methods. We use LRP in this work owing to its popularity, but in principle, the heatmap extraction module can incorporate any other method widely in use today. LRP is a backward propagation based technique relying on the relevance conservation principle across each neuron in each layer. The output is a set of relevance scores that can be attributed to a pixel wise decomposition of the input image. Heatmap-based explainability techniques have also been used in conjunction with clustering, in the context of discovering model strategies for classification, and disparate areas such as differential privacy~\cite{Lapuschkin2019UnmaskingCH, Chen2018DetectingBA, Schulth2022DetectingBP}.


==> ExMap-3/sec/3_finalcopy.tex <==
\section{Worst Group Robustness}
In this section, we provide notation and brief background of the group robustness problem. We are given a dataset \(D\) with image-label pairs being defined as \(D = \{(x_i, y_i)\}_{i=1}^{N}\), where \(x_i\) represents an image, \(y_i\) is its corresponding label, and \(N\) is the number of pairs in the dataset. The model's prediction for an image \(x\) is \(y_{\text{pred}} = \hat{f}(x)\). The cross-entropy loss for true label \(y\) and predicted label \(y_{\text{pred}}\) is given by \(L(y, y_{\text{pred}}) = -\sum_{c=1}^{C} y_c \log(y_{\text{pred},c})\), where \(C\) is the number of classes. Then, an ERM 
classifier simply minimizes the average loss over the training data:
\begin{equation}
\hat{f} = \arg\min_{f} \frac{1}{N} \sum_{i=1}^{N} L(y_i, f(x_i))
\end{equation}
where \(\hat{f}\) is the model obtained after training. Next, given the validation data $D$, we assume that for the class label set $L = \{c_1, c_2, ..., c_k\}$ there exists a corresponding spurious attribute set $A = \{a_1, a_2, ..., a_m\}$, such that the group label set $G: L \bigtimes A$. For example, in CelebA, typically $a:$ Gender (Male/Female), and $c$: Blonde Hair (Blonde/Not Blonde). In this case $L = \{0,1\}$, and $A = \{0, 1\}$. Then, the optimization can be described as the worst-expected loss over the validation set, conditioned on the group labels and the spurious attributes:

\begin{equation}
\hat{f}^* = \arg\min_{f} \max_{(c_i, a_j) \in G} \mathbb{E}_{(x, y) \in D} [L(y, f(x)) | c_i, a_j]
\end{equation}

As discussed before, recent works aim to design strategies over the (base) trained model to minimize this objective. For example, JTT collects an error set from the training data, and then upweights misclassified examples during the second training phase. DFR reweights the features responsible for misclassifications during the first phase in its finetuning stage. Note, however, that both these methods rely on the validation set \textit{group labels} $G_{val}$ to finetune the network. We consider the case where $G_{train} = \phi$ and $G_{val} = \phi$. We do not have access to group labels, and must therefore infer pseudo-labels in an unsupervised manner so that existing group robustness methods can be used.
% We do not have access to either the training or validation group labels. The task is to infer \textit{pseudo-labels} in an unsupervised manner that can then be used in these training strategies.  

\begin{figure*}[t]
    \centering    % Second image
    %\vspace{-5cm}
    \includegraphics[width=\linewidth]{images/exmap.pdf}
    %\vspace{-3cm}
    \caption{Our Proposed Method: ExMap  facilitates group-robustness by extracting explainability heatmaps from the frozen base ERM model for the validation data (A). These heatmaps are then clustered (B) to obtain pseudo-labels for the underlying groups, which are subsequently chosen for the retraining strategy (C).}\vspace{-3mm}
    \label{fig:exmap}
\end{figure*}

==> ExMap-3/sec/4_method.tex <==
\section{Leveraging Explainability Heatmaps for Group Robustness -- ExMap}

In this section, we describe ExMap, an intuitive and efficient approach for unsupervised group robustness to spurious correlations. ExMap is a two-stage method, illustrated in Figure~\ref{fig:exmap}. In the first stage, we extract explainability heatmaps for the model predictions. In the second stage, we cluster the heatmaps to generate pseudo-labels. These pseudo-labels can then be used on any off-the-shelf group robustness strategy in use today. In our work, we demonstrate the strategy agnostic nature of ExMap by running it on two popular strategies - JTT and DFR.

\subsection{Explainability Heatmaps}
We use LRP \cite{Bach2015OnPE} in this stage to generate pixel attributions in the input space. This allows us to focus only on the relevant features for the task. Specifically, given the validation data \(D_{val} = \{(x_i, y_i)\}_{i=1}^{M}\), we use pixel wise relevance score  $r_x = (\mathcal{LRP}(x)) \forall x \in D_{val}$. Specifically, for each data point $x$, the relevance score is defined on a per-neuron-per layer basis. For an input neuron $n_k$ at layer $k$, and an output neuron $n_l$ at the following layer $l$, the relevance score $R_{k}$ is intuitively a measure of how much this particular input $n_k$ contributed to the output value $n_l$: 
\begin{equation}
     R_{k} = \sum_{l: k \xrightarrow{}l}\frac{z_{kl}}{z_l + \varepsilon \cdot \sign(z_{l})} 
     \label{eq:lrp}
\end{equation} 
%\vspace{-0.1cm}
where $z_{l} = n_kw_{kl}$ for the weight connection $w_{kl}$. $R_k$ is computed for all the neurons at layer $k$, and backpropagated from the output layer to the input layer to generate pixel level relevance scores $r_x$ for each data input $x$. We can thus build the heatmap set $R = \{r_x | x \in D_{val}\}$. This process is summarized in Algorithm ~\ref{algo:exmap}. 

\begin{figure*}[t]
    \centering
  \includegraphics[width=1.0\textwidth, trim={2cm 0 13cm 0},clip]{images/dataset.pdf}\vspace{-2mm}
    \caption{The datasets used in our work, visualized with respect to the class labels, and the shortcuts $s$. For the complete list of datasets and more details, please refer to the supplementary material.}\vspace{-4mm}
    \label{fig:datasets}
\end{figure*}
\label{sec:method}

\begin{algorithm}[t]
\caption{Generating Pseudo-labels using G-ExMap}
\label{algo:exmap}
\begin{algorithmic}[1]
\State \textbf{Input:} Dataset \(D_{val}\), ERM Model \(\mathcal{M}\), DataLoader \(\mathcal{L}\)
\State \textbf{Output:} Pseudo-labels \(\hat{G}\)

\Procedure{GeneratePseudoLabels}{$D, \mathcal{M}, \mathcal{L}$}

    \State \(R \gets \emptyset\)  
    \Comment{Initialize heatmap set}
    
    \For{each batch \(x\) in \(\mathcal{L}\)}
        \State \(\text{pred} \gets \arg\max_{i} \mathcal{M}(x)_i\)
        
        \For{each layer \(k, l\)}
            %\State \(a_k\): Activation of neuron $a$, layer $k$.
            \State Compute \(z_{l} \gets n_kw_{kl}\)
        \EndFor
        \State Compute LRP relevance \(r_x\) for \(x\) using Eq. \ref{eq:lrp}
        
        \State Add \(r_x\) to \(R\)
    \EndFor
    \State Cluster \(R\) using G-ExMap method:
    \State \(\hat{A} \gets \text{Cluster}(R) \)
    \Comment{Estimated spurious labels}

    \State Combine class labels $L$ with $\hat{A}$
    \[ \hat{G} \gets L \times \hat{A} \]
    
    \State \Return \( \text{Pseudo-labels } \hat{G} \)

\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Clustering}

In the second stage, we cluster the LRP representations from the first stage. The intuition here is that over the data, the heatmaps capture the different strategies undertaken by the model for the classification task \cite{Lapuschkin2019UnmaskingCH}. The clustering module helps identify dominant model strategies used for the classification task. By identifying such strategies and resampling in a balanced manner, ExMap guides the model to be less reliant on the dominant features across the data, i.e. the spurious features. The heatmaps serve as an effective proxy to describe model focus areas. We have two options in choosing how to cluster: Local-ExMap (L-ExMap), where we cluster heatmaps on a per-class basis, and Global-ExMap (G-ExMap), where we cluster all the heatmaps at once, and segment by class labels. We present the G-ExMap results in this paper, owing to better empirical results. 

Specifically, given the Heatmap set $R$ as described in Algorithm \ref{algo:exmap}, the estimated spurious labels are generated by the global clustering method, $\hat{A} = \text{Cluster}(R)$
where \(\text{Cluster (.)}\) represents a clustering function.
Now, given class label set $L$ and estimated spurious label set $\hat{A}$, we can generate our pseudo-\textit{group} label set $\hat{G} = L \bigtimes A$ by selecting each $a_i \in \hat{A}$, and each $c_k \in L$, to create $\{c_k, a_i\}$ $\forall k, i$.
% \begin{figure}[t]
%     \centering
%   \includegraphics[width=\textwidth]{ExMap/images/datasets.pdf}
%     %\vspace{-3cm}
%     \caption{The Clever Hans effect: Model picks up the spurious watermark as the classification rule instead of focusing on relevant object part. }
%     \label{fig:datasets}
% \end{figure}
% \label{sec:method}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{ExMap/images/datasets.pdf}
%     %\vspace{-3cm}
%     \caption{The Clever Hans effect: Model picks up the spurious watermark as the classification rule instead of focusing on relevant object part. }
%     \label{fig:datasets}
% \end{figure}
 In principle, it doesn't matter what clustering method we use, but that the clustering process itself outputs useful pseudo-labels. For our work, we leverage spectral clustering with an eigengap heuristic, inspired by SPRAY \cite{Lapuschkin2019UnmaskingCH}. Later, we show that the choice of the clustering method does not have a significant effect on the results. The outputs, which are the pseudo group labels for the validation data $D_{val}$, can now be used as labels in lieu of ground truth labels to train any group robustness strategy in use. Note how in principle, \textit{any} method that uses group labels (training or validation) would benefit from this approach. To apply this to the training set $D$, one would simply repeat Algorithm \ref{algo:exmap} on $D$. In this work, we apply ExMap to two common group robustness strategies - JTT \cite{Liu2021JustTT} and DFR \cite{Kirichenko2022LastLR}. Thus, we demonstrate the strategy-agnostic nature of our approach that can be applied to any off-the-shelf method using group labels today. 





==> ExMap-3/sec/5_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

%\end{document}
% \begin{table*}[!t]
%     \centering
%     \setlength{\tabcolsep}{12pt}
%     \resizebox{0.9\linewidth}{!}{\begin{tabular}{lcllll}
    
%         \toprule
%         \textbf{Methods} & \textbf{Group Info} & \multicolumn{2}{c}{\textbf{Waterbirds}} & \multicolumn{2}{c}{\textbf{CelebA}} \\
%         \cmidrule(lr){3-4} \cmidrule(lr){5-6}
%         & Train/Val & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) \\
%         \midrule
%         \rowcolor{gray!25}
%         Base (ERM) & \xmark/\xmark & 76.8 & 98.1 & 41.1 & 95.9\\
%         \hline
%         % CnC & \xmark/\cmark & - & - & & & \\
%         % SSA & \xmark/\cmark\cmark & - & - & & & \\
%         % SUBG & \cmark/\cmark & - & - & & & \\
%         \rowcolor{gray!25}
%         Group DRO & \cmark/\cmark & 91.4 & 93.5 & 88.9 & 92.9 \\
%         \rowcolor{gray!25}
%         EIIL & \cmark/\cmark & 87.3 & 93.1 & 81.3 & 89.5 \\
%         % DISC & \xmark/\cmark & 88.7 & 93.8 & - & - \\
%         \rowcolor{gray!25}
%         BARACK & \cmark/\cmark & 89.6 & 94.3 & 83.8 & 92.8 \\
%         \rowcolor{gray!25}
%         CVar DRO  & \xmark/\cmark & 75.9 & 96.0 &  64.4 & 82.5 \\
%         \rowcolor{gray!25}
%         LfF  & \xmark/\cmark & 78.0 & 91.2 &  77.2 & 85.1\\
%         \rowcolor{gray!25}
%         JTT  & \xmark/\cmark & 86.7 & 93.3 & 81.1 & 88.0 \\
%         \rowcolor{gray!25}
%         DFR & \xmark/\cmark & 92.1 & 96.7 & 86.9 & 91.1 \\ 
         
         
%         \hline
%         GEORGE (gDRO) & \xmark/\xmark & 76.2 & 95.7 & 53.7 & 94.6 \\
%         CVar DRO  & \xmark/\xmark & 62.0 & 96.0 &  36.1 & 82.5 \\
%         LfF  & \xmark/\xmark & 44.1 & 91.2 &  24.4 & 85.1 \\
%         JTT  & \xmark/\xmark & 62.5 & 93.3 & 40.6 & 88.0 \\
%         DivDis* & \xmark/\xmark & 81.0 & - & 55.0 & - \\ 
%         MaskTune & \xmark/\xmark & 86.4 & 93.0 & 78.0 & 91.3 \\
%         GEORGE (DFR) & \xmark/\xmark & 91.7 & 96.5 & 83.3 & 89.2 \\ 
%         DFR+ExMap (ours) & \xmark/\xmark & \textbf{92.5} & 96.0 & \textbf{84.4} & 91.8 \\
%         % G-XFR (ours) & \xmark/\xmark\xmark & 63.3$_{\pm1.0}$ & 96.8$_{\pm0.2}$ & 84.7$_{\pm1.0}$ & 88.5$_{\pm1.3}$ & 77.8$_{\pm0.9}$ & 92.8$_{\pm0.0}$\\
%         \bottomrule
%     \end{tabular}}
%     \caption{Worst group and mean accuracy on the test sets of the different datasets. The Group Info column showcases for each method whether group labels are used for that split of the data (\xmark = does not use group labels, \cmark = uses group labels). We report the average results over 5 runs after hyperparameter tuning. Gray rows represent supervised approaches. *DivDis does not report mean test accuracy results.}
%     \label{tab:mainresult}
% \end{table*}
% \begin{table*}[!t]
%     \centering
%     \resizebox{0.9\linewidth}{!}{\begin{tabular}{lcllllll}
%         \toprule
%         \textbf{Methods} & \textbf{Group Info} & \multicolumn{2}{c}{\textbf{C-MNIST}} & .\multicolumn{2}{c}{\textbf{Urbancars (BG)}} & \multicolumn{2}{c}{\textbf{Urbancars (CoObj)}} \\
%         \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%         & Train/Val & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) \\
%         \midrule
%         \rowcolor{gray!25}
%         Base (ERM) & \xmark/\xmark & 39.6 & 99.3 & 55.6 & 90.2 & 50.8 & 92.7\\
%         % $_{Tr}^{Val}$
%         \rowcolor{gray!25}
%         DFR & \xmark/\cmark & 74.2 & 93.7 & 77.5 & 81.0 & 84.7 & 88.2 \\ 
%         \hline

%         GEORGE (DFR) & \xmark/\xmark & 71.7 & 95.2 & 69.1 & 83.6 & 76.9 & 91.4 \\
         
%         DFR+ExMap (ours) & \xmark/\xmark & \textbf{72.5} & 94.9 & \textbf{71.4} & 93.2 & \textbf{79.2} & 93.2
%         \\
%         \bottomrule
%     \end{tabular}}
%     \caption{Worst Group accuracy and mean accuracy on C-MNIST, Urbancars (BG), and Urbancars(CoObj). We use GEORGE as the baseline, since both GEORGE and ExMap significantly outperform other unsupervised methods on Waterbirds and CelebA. Gray rows represent supervised approaches.}
%     \label{tab:mainresult-george}
% \end{table*}

% \begin{table*}[!t]
%     \centering
%     \resizebox{0.9\linewidth}{!}{%
%     \begin{tabular}{lcllllll}
%         \toprule
%         \textbf{Methods} & \textbf{Group Info} & \multicolumn{2}{c}{\textbf{C-MNIST}} & \multicolumn{2}{c}{\textbf{Urbancars (BG)}} & \multicolumn{2}{c}{\textbf{Urbancars (CoObj)}} \\
%         \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%         & Train/Val & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) \\
%         \midrule
%         \rowcolor{gray!25}
%         Base (ERM) & \xmark/\xmark & 39.6 & 99.3 & 55.6 & 90.2 & 50.8 & 92.7\\
%         \rowcolor{gray!25}
%         DFR & \xmark/\cmark & 74.2 & 93.7 & 77.5 & 81.0 & 84.7 & 88.2 \\ 
%         \hline
%         GEORGE (DFR) & \xmark/\xmark & 71.7 & 95.2 & 69.1 & 83.6 & 76.9 & 91.4 \\
%         DFR+ExMap (ours) & \xmark/\xmark & \textbf{72.5} & 94.9 & \textbf{71.4} & 93.2 & \textbf{79.2} & 93.2 \\
%         \bottomrule
%     \end{tabular}}
%     \caption{Worst Group accuracy and mean accuracy on C-MNIST, Urbancars (BG), and Urbancars(CoObj). We use GEORGE as the baseline, since both GEORGE and ExMap significantly outperform other unsupervised methods on Waterbirds and CelebA. Gray rows represent supervised approaches.}
%     \label{tab:mainresult-george}
% \end{table*}

In this section we first present the datasets, baselines, and experimental setup. Next, we present the results and discussion\footnote{A discussion of the limitations and societal impact can be found in the supplementary material.}.

\paragraph{Datasets}

We use CelebA \cite{liu2015faceattributes}, Waterbirds \cite{Sagawa2019DistributionallyRN, Zhou2016PlacesAI, WahCUB_200_2011}, C-MNIST \cite{Arjovsky2019InvariantRM}, and Urbancars \cite{Li2022AWD}. In CelebA, the class label to be predicted is hair colour (Blonde/Not Blonde), and the spurious attribute is gender (Male/Female). For Waterbirds, the class label is the bird type (waterbird/landbird), and the spurious attribute is the background (land/water). In C-MNIST, the class label is if the number is smaller than or equal to four. Any number lesser than or equal to four is assigned blue, while all numbers greater than four are assigned the color red, with a correlation of 99\%. Thus, the spurious attribute is the color. 
For Urbancars, the class label is the car type (country/urban), and the spurious attributes are the background and co-occuring object (both country/urban). We create two variants of Urbancars: The first variant is Urbancars (BG), where only the background object is the spurious attribute. The second variant is Urbancars (CoObj), where the co-occuring object is the spurious attribute. We present single shortcut results on CelebA, Waterbirds, C-MNIST, Urbancars (BG) and Urbancars (CoObj). For the multiple shortcut setting, we use the original UrbanCars dataset with both shortcuts \cite{Li2022AWD}. An overview over the considered datasets can be found in Figure \ref{fig:datasets}. We present more dataset details in the supplementary. 

\paragraph{Baselines}

We use the unsupervised approaches DivDis, MaskTune, and two variants of GEORGE (with gDRO and DFR) as the baselines in our work. We also adapt LfF, JTT, and CVar DRO to the unsupervised setting as additional baselines. We train the ERM model using an Imagenet-pretrained Resnet-50, and use the open source implementations of the baselines to generate our results. Specifically, we implement GEORGE(DFR), ExMap, and JTT. Remaining results are reported from \cite{Taghanaki2022MaskTuneMS}, \cite{Liu2021JustTT}, and \cite{Lee2023DiversifyAD}. 

\paragraph{Setup}

We make sure to use the same hyperparameters from the baseline papers to reproduce the results. We utilise a composite of LRP rules to get the explainability heatmaps as recommended by \cite{Montavon2019LayerWiseRP, Kohlbrenner2019TowardsBP}. Following their recommendations we use LRP-$\epsilon$ for the dense layers near the output of the model with small epsilon ($\epsilon \ll 1$), followed by LRP-$\gamma$ for the convolutional layers.

For the spectral clustering, we use the affinity matrix, and cluster-QR \cite{Schulth2022DetectingBP} to perform the clustering. The eigengap heuristic is applied to the 10 smallest eigenvalues of the Laplacian matrix to select the number of significant clusters to use. We demonstrate later that using a simpler clustering approach such as k-means can also emit reasonable results. For more details on the affinity matrix, clustering and pseudo-label generation, please see the supplementary. 
%\vspace{-0.5cm}
\begin{table*}[!t]
    \centering
    \setlength{\tabcolsep}{12pt}
    \resizebox{0.9\linewidth}{!}{\begin{tabular}{lcllll}
    
        \toprule
        \textbf{Methods} & \textbf{Group Info} & \multicolumn{2}{c}{\textbf{Waterbirds}} & \multicolumn{2}{c}{\textbf{CelebA}} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6}
        & Train/Val & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) \\
        \midrule
        Base (ERM) & \xmark/\xmark & 76.8 & 98.1 & 41.1 & 95.9\\
        \hline
        % CnC & \xmark/\cmark & - & - & & & \\
        % SSA & \xmark/\cmark\cmark & - & - & & & \\
        % SUBG & \cmark/\cmark & - & - & & & \\
        \rowcolor{gray!25}
        Group DRO & \cmark/\cmark & 91.4 & 93.5 & 88.9 & 92.9 \\
        \rowcolor{gray!25}
        EIIL & \cmark/\cmark & 87.3 & 93.1 & 81.3 & 89.5 \\
        % DISC & \xmark/\cmark & 88.7 & 93.8 & - & - \\
        \rowcolor{gray!25}
        BARACK & \cmark/\cmark & 89.6 & 94.3 & 83.8 & 92.8 \\
        \rowcolor{gray!25}
        CVar DRO  & \xmark/\cmark & 75.9 & 96.0 &  64.4 & 82.5 \\
        \rowcolor{gray!25}
        LfF  & \xmark/\cmark & 78.0 & 91.2 &  77.2 & 85.1\\
        \rowcolor{gray!25}
        JTT  & \xmark/\cmark & 86.7 & 93.3 & 81.1 & 88.0 \\
        \rowcolor{gray!25}
        DFR & \xmark/\cmark & 92.1 & 96.7 & 86.9 & 91.1 \\ 
         
         
        \hline
        GEORGE (gDRO) & \xmark/\xmark & 76.2 & 95.7 & 53.7 & 94.6 \\
        CVar DRO  & \xmark/\xmark & 62.0 & 96.0 &  36.1 & 82.5 \\
        LfF  & \xmark/\xmark & 44.1 & 91.2 &  24.4 & 85.1 \\
        JTT  & \xmark/\xmark & 62.5 & 93.3 & 40.6 & 88.0 \\
        DivDis* & \xmark/\xmark & 81.0 & - & 55.0 & - \\ 
        MaskTune & \xmark/\xmark & 86.4 & 93.0 & 78.0 & 91.3 \\
        GEORGE (DFR) & \xmark/\xmark & 91.7 & 96.5 & 83.3 & 89.2 \\ 
        DFR+ExMap (ours) & \xmark/\xmark & \textbf{92.5} & 96.0 & \textbf{84.4} & 91.8 \\
        % G-XFR (ours) & \xmark/\xmark\xmark & 63.3$_{\pm1.0}$ & 96.8$_{\pm0.2}$ & 84.7$_{\pm1.0}$ & 88.5$_{\pm1.3}$ & 77.8$_{\pm0.9}$ & 92.8$_{\pm0.0}$\\
        \bottomrule
    \end{tabular}}
    \caption{Worst group and mean accuracy on the test sets of the different datasets. The Group Info column showcases for each method whether group labels are used for that split of the data (\xmark = does not use group labels, \cmark = uses group labels). We report the average results over 5 runs after hyperparameter tuning. Gray rows represent supervised approaches. *DivDis does not report mean test accuracy results.}
    \label{tab:mainresult}
\end{table*}

\begin{table*}[!t]
    \centering
    \resizebox{0.9\linewidth}{!}{%
    \begin{tabular}{lcllllll}
        \toprule
        \textbf{Methods} & \textbf{Group Info} & \multicolumn{2}{c}{\textbf{C-MNIST}} & \multicolumn{2}{c}{\textbf{Urbancars (BG)}} & \multicolumn{2}{c}{\textbf{Urbancars (CoObj)}} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
        & Train/Val & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) & WGA(\%)\color{Green}{$\uparrow$} & Mean(\%) \\
        \midrule
        Base (ERM) & \xmark/\xmark & 39.6 & 99.3 & 55.6 & 90.2 & 50.8 & 92.7\\
        \rowcolor{gray!25}
        DFR & \xmark/\cmark & 74.2 & 93.7 & 77.5 & 81.0 & 84.7 & 88.2 \\ 
        \hline
        GEORGE (DFR) & \xmark/\xmark & 71.7 & 95.2 & 69.1 & 83.6 & 76.9 & 91.4 \\
        DFR+ExMap (ours) & \xmark/\xmark & \textbf{72.5} & 94.9 & \textbf{71.4} & 93.2 & \textbf{79.2} & 93.2 \\
        \bottomrule
    \end{tabular}}
    \caption{Worst Group accuracy and mean accuracy on C-MNIST, Urbancars (BG), and Urbancars (CoObj). We use GEORGE as the baseline, since both GEORGE and ExMap significantly outperform other unsupervised methods on Waterbirds and CelebA. Gray rows represent supervised approaches.}
    \label{tab:mainresult-george}
\end{table*}

\subsection{Results: Single Shortcut}

In Table \ref{tab:mainresult} we present the single shortcut results for the datasets. First, we note that with no supervision, ExMap based DFR improves significantly upon ERM. Second, we note the improved performance of ExMap based DFR over the unsupervised baselines, including GEORGE, our closest baseline.
Further, since the DFR-based GEORGE and ExMap significantly outperforms the other baselines, we present results comparing these two methods on C-MNIST, Urbancars (BG) and Urbancars (CoObj) in Table \ref{tab:mainresult-george}. In both tables, we demonstrate the superiority of clustering heatmaps to generate pseudo-labels instead of the raw features as in GEORGE. These results also show that the groups inferred by ExMap are indeed useful for worst group robustness to spurious correlations. Third, we note the gap in performance between DFR and ExMap based DFR. Since the former uses validation labels, we expect an increased accuracy, but we can report better performance on Waterbirds, and within 3\%\, 2\%\, 8\%\, and 6\%\ of the DFR results on the remaining datasets. On CelebA, our results are within 5\%\ of Group-DRO, which demonstrates the best overall results. However, note that Group-DRO is a fully supervised approach, using labels from both the training and validation sets. For all datasets, we are able to outperform GEORGE, our closest baseline. As discussed before, while mean accuracy is not the appropriate metric to track in the group robustness setting (ERM has the best overall mean accuracy but the worst overall worst group accuracy), we can still confirm that ExMap based DFR does not witness significant drops in performance. 

\subsection{Results: Multiple Shortcuts}

Here, we present the results on the UrbanCars data, which contains multiple shortcuts in the images - the background and the co-occurring object in the image. This dataset was introduced in the recent work on multiple shortcut mitigation \cite{Li2022AWD}, where the authors show that mitigating one shortcut may lead to a reliance on another shortcut in the data, rendering the single shortcut setting incomplete (the Whac-a-Mole problem). The authors introduce a new set of metrics for the task - The \textbf{BG Gap}, which is the drop in accuracy between mean and cases when only the background is uncommon, the \textbf{CoObj Gap} which is the drop in accuracy between mean and cases when only the co-occurring object is uncommon, and the \textbf{BG+CoObj Gap}, the drop when both the background and the co-occurring object are uncommon. A mitigation strategy should witness a smaller drop from the original accuracy when compared to others. In Table \ref{tab:multishortcut}, we present the ExMap based DFR results with respect to DFR, ERM, and GEORGE(DFR). We also present results of three variants of DFR: DFR (Both), which is retraining on the original UrbanCars data with both shortcuts. DFR(BG) retrains on UrbanCars with only the background shortcut, and DFR(CoObj) retrains with only the co-occuring object shortcut. Red values indicate an increase in gap when compared to ERM, which is undesirable (the Whac-A-Mole dilemma). Note that the first three DFR methods have access to the group labels, while GEORGE and ExMap do not. Table \ref{tab:multishortcut} demonstrates some important results: First, that DFR + ExMap consistently posts lower drops than the base ERM model. Second, that ExMap does not witness an increase in gap on any of the metrics compared to ERM, unlike GEORGE(DFR), which exhibits the Whac-A-Mole dilemma for the CoObj Gap. Finally, the DFR variants exhibit the Whac-A-Mole dilemma: For a DFR variant retrained on a particular shortcut, the reliance on that shortcut is mitigated (e.g. DFR (BG) mitigates the BG Gap), but the other shortcut reliance is exacerbated (DFR (BG) exhibits a higher CoObj Gap than ERM).
Note that DFR uses the validation group labels, and hence will be more useful in mitigating shortcuts than our unsupervised setting. In fact, as demonstrated in \cite{Li2022AWD}, training separate classifiers for each shortcut is the best approach to mitigating multiple shortcuts, which explains DFR's best overall results. However, this setting assumes availability to the shortcut labels, which ExMap does not assume. Yet, it demonstrates a robust performance for the multi-shortcut setting even in the unsupervised setting, outperforming GEORGE, its closest unsupervised competitor. 

\begin{table}[tbp]
\centering
\resizebox{.5\textwidth}{!}{\begin{tabular}{lllc}
\toprule
\textbf{Method} & \textbf{BG Gap} \color{Green}{$\uparrow$} & \textbf{CoObj Gap} \color{Green}{$\uparrow$} & \textbf{BG+CoObj Gap} \color{Green}{$\uparrow$}\\
\midrule
ERM & -8.2 & -14.2 & -69.0 \\
\rowcolor{gray!25}
DFR (Both) & -4.6 & -5.4 & -14.2 \\
\rowcolor{gray!25}
DFR (BG) & -0.3 & -29.2 (\textcolor{red}{$\times$ 2.06}) & -33.2 \\
\rowcolor{gray!25}
DFR (CoObj) & -16.3 (\textcolor{red}{$\times$ 1.99}) & -0.5 & -19.1 \\
\midrule
GEORGE (DFR) & -7.0 & -15.4 (\textcolor{red}{$\times$1.08}) & -63.4 \\
DFR+ExMap (ours) & \textbf{-5.9} & \textbf{-9.9} & \textbf{-30.7} \\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{Multiple Shortcuts on UrbanCars. Red values indicate the Whac-A-Mole dilemma: Mitigating one shortcut exacerbates reliance on the other (compared to ERM). ExMap proves to be the most robust in this setting, and outperforms GEORGE, its direct unsupervised counterpart.}\vspace{-4mm}
\label{tab:multishortcut}
\end{table}
\begin{figure}[!t]
\centering
%\vspace{-1cm}
\includegraphics[width=\linewidth]{images/heatmaps.pdf}
    %\vspace{-1.3cm}
    \caption{ERM and ExMap Heatmaps - Left: The Input images. Middle: ERM model explanations. Right: Improved group robustness using ExMap. Our method helps improve the focus on relevant attributes, in turn improving the pseudo-label estimation for retraining.}\vspace{-3mm}
    \label{fig:heatmaps}
\end{figure}





%\end{document}

==> ExMap-3/sec/6_analysis.tex <==
%\vspace{-0.3cm}
\section{Analysis}
\label{sec:analysis}
%\vspace{-1cm}
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/celeba.pdf}
    \vspace{-0.6cm}
    \caption{ExMap Heatmaps on CelebA: Each entry represents a group. The positive and negative attributions help interpret which features the model considers spurious (Blue), and which features are helpful (Red).}\vspace{-0.3cm}
    
    \label{fig:celeba}
\end{figure}
%\vspace{-1cm}
In this section, we present analysis and ablations along five axes: First, we demonstrate how the clustering of heatmaps is more useful than the clustering of features. Second, we demonstrate the usefulness of the ExMap representations when compared to ERM with respect to the classification task. Third, we provide more insight into what the learned clusters by ExMap capture in the data. Fourth, we demonstrate that ExMap is robust to the choice of clustering method, by performing an ablation on the clustering method using k-means instead of spectral clustering. Finally, to demonstrate that ExMap is strategy-agnostic, we use JTT as a retraining strategy using ExMap pseudo-labels, and are able to demonstrate robust performance with respect to JTT trained on true validation labels. 

\subsection{The benefit of heatmaps over features}
In this section we add more insight into why leveraging heatmaps for worst group robustness is more useful over features, as for example done in GEORGE. Specifically, we illustrate how heatmap based clustering mitigates reliance on the image background, the spurious attribute in the Waterbirds dataset. The results illustrate a common intuition - Explainability heatmaps highlight only the features relevant for prediction, ignoring those that are not. 
\paragraph{Circumventing background reliance}

Here, we present results on Waterbirds with the spurious attribute, i.e. background, removed. We call this variant Waterbirds (FG-Only), following \cite{Kirichenko2022LastLR}. Please refer to the supplementary section for examples. An effective group robustness method would not witness a sharp drop in test accuracy if the model does not rely on the background. In Table \ref{tab:fgonly}, we present these results. 

\begin{table}[t]
    \centering
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lccc}
        \toprule
        \textbf{Methods} & \textbf{Mean (FG-Only \%)} & \textbf{Mean (\%)} & \textbf{Drop}
        \color{Green}{$\downarrow$} \\
        \midrule
        ERM & 44.2 & 98.1 & 53.9 \\
        \rowcolor{gray!25}
        DFR & 64.7 & 94.6 & 29.9 \\
        GEORGE (DFR) & 73.2 & 96.5 & 23.3 \\
        DFR+ExMap (ours) & 78.5 & 96.0 & \textbf{17.5} \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}\caption{Waterbirds (FG-Only). All methods exhibit a reliance on the background shortcut in Waterbirds, but ExMap posts the lowest drop, demonstrating its robustness.}\vspace{-3mm}
    \label{tab:fgonly}
\end{table}
%\vspace{-3cm}
% \begin{figure}[t]
%     \centering
%     %\vspace{-1cm}
%     % \begin{adjustbox}{width=.7\textwidth}
%     %     \includegraphics{ExMap/images/fgonly.pdf}
%     % \end{adjustbox}
%     \includegraphics[width=0.625\linewidth]{ExMap/images/fgonly.pdf}
%     %\vspace{-1.5cm}
%     \caption{Waterbirds (FG-Only). All methods exhibit a reliance on the background shortcut in Waterbirds, but ExMap posts the lowest drop, demonstrating its robustness.}
%     \label{fig:fgonly}
% \end{figure}


We can clearly see that the heatmap clustering strategy mitigates the background reliance better than the feature based clustering strategy of GEORGE (lowest drop among all methods). This is also intuitive as the heatmap attributions focus on only the relevant features for prediction, discarding the rest (see Figure \ref{fig:heatmaps}).

% \paragraph{Sensitivity to number of clusters}

% The heatmap based clustering strategy with SpRay is also useful when it comes to choosing the number of clusters. As we show in Figure \ref{fig:sensi}, the clustering strategy with features is far more sensitive to the number of clusters chosen. In the case of GEORGE, while good worst group robustness can be achieved, it is important to choose the correct number of clusters \cite{Sohoni2020NoSL}. In the case of ExMap, since the eigengap heuristic automatically chooses the number of clusters, we are more robust to the choice of clusters. Intuitively, this follows from the previous results on background reliance - Focusing only on relevant features leads to less noise in the clustering approach, leading to stable results. 

% \begin{figure}[h]
%     \centering
%     % First image
%     \includegraphics[width=.35\textwidth]{ExMap/images/sensi_exmap.png}
%     \hspace{0.02\textwidth} % Spacing between images, adjust if needed
%     % Second image
%     \includegraphics[width=.35\textwidth]{ExMap/images/sensi_george.png}
%     \caption{Sensitivity to number of clusters. ExMap (Above) is more robust to the choice than GEORGE (Below).}
%     \label{fig:sensi}
% \end{figure}
% \vspace{-0.35cm}

\subsection{Qualitative Analysis}
\paragraph{ExMap improves explanations upon retraining}
% \todo{This section title needs to be modified and focused more towards exmap}

We visualize the heatmaps and predictions of ERM and Exmap based DFR in Figure \ref{fig:heatmaps}. This is an image of the Waterbirds dataset that ERM misclassifies. This is reflected on the heatmap, as ERM fails to capture the relevant features. On the other hand, ExMap based DFR correctly classifies the image and focuses on the correct object region of interest (bird), instead of the spurious attribute (background).

\paragraph{ExMap improves Model Strategy}

\begin{table}[!t]
    \centering
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcll}
        \toprule
        \textbf{Methods} & \textbf{Group Info} & \textbf{WGA(\%)} \color{Green}{$\uparrow$} & \textbf{Mean(\%)} \color{Green}{$\uparrow$} \\
        \midrule
        Base (ERM) & \xmark/\xmark & 76.8 & 98.1 \\
        % \hline
        \rowcolor{gray!25}
        DFR & \xmark/\cmark & 92.1 & 96.7 \\  
        \hline
        DFR+ExMap (SC) & \xmark/\xmark & 92.6 & 96.0 \\
        DFR+ExMap (KMeans) & \xmark/\xmark & 92.5 & 95.9 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}
    \caption{Worst group accuracy and mean accuracy on Waterbirds with two different clustering methods - kmeans and Spectral.}\vspace{-5mm}
    \label{tab:ablate1}
\end{table}

In Figure \ref{fig:celeba}, each entry represents a particular group. The positive and negative relevance scores correspond to the features that the model considers relevant and spurious respectively. ExMap uncovers the strategy used to make the prediction: In all four groups, we see ExMap helps the model uncover the hair color as a strategy. In fact, in Group 4, the model also learns that the facial features (Gender) are \textit{negatively} associated with the prediction task (Hair Color), which is what we desire from our method. The model has learned the shortcut between man and not-blonde hair, hence ExMap uncovers the negative relevance in the face, effectively uncovering this shortcut. These examples impart a notion of interpretability to our results, as we are able to explain why the model made a particular prediction, and what shortcuts are uncovered.


% \begin{figure}[t]
%     \centering
%     % First image
%     \includegraphics[width=.15\textwidth]{ExMap/images/tsne1.png}
%     \hspace{0.02\textwidth} % Spacing between images, adjust if needed
%     % Second image
%     \includegraphics[width=.15\textwidth]{ExMap/images/tsne2.png}
%     \caption{t-SNE plot of CelebA heatmaps in 2D coloured with ground truth groups. Left: class $y=0$, Right: class $y=1$. It is impossible to recover the ground truth labels here.}
%     \label{fig:tsne_celeba}
% \end{figure}

\subsection{Ablation Analysis}
\paragraph{Robustness to choice of clustering method}
Our proposed method does not depend on any particular clustering algorithm. Although we used spectral clustering, one can also use the simpler K-means \cite{kmeans} to capture the clusters for pseudo-labelling. In Table \ref{tab:ablate1}, we present the results on Waterbirds. We are able to demonstrate that there is no significant difference in the worst group robustness performance for the clustering method we choose\footnote{Note, empirical results illustrated that k-means results were robust to the number of clusters, $K$, given that $K$ was chosen sufficiently large.}. Both improve upon the base ERM and DFR models, and hence, both are useful. Thus, ExMap is more about demonstrating the usefulness of a heatmap clustering pseudo-labelling module rather than the specifics of the clustering method itself. 

\paragraph{Robustness to choice of learning strategy}
All the results presented until now focus on the DFR backbone for shortcut mitigation. We mention previously that ExMap is strategy-agnostic, meaning that it can be applied to any off-the shelf method in use today. In Table \ref{tab:ablate2}, we show the results after applying ExMap to the JTT method on Waterbirds. We demonstrate similar performance to using JTT (originally uses validation labels) simply by using the pseudo labels proposed by ExMap. Additionally, we are able to improve over ERM's poor worst group accuracy as well. 

% \begin{table}[!t]
%     \centering
%     \resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{lcll}
%         \toprule
%         \textbf{Methods} & \textbf{Group Info} & \textbf{WGA(\%)} & \textbf{Mean(\%)} \\
%         \midrule
%         Base (ERM) & \xmark/\xmark & 41.1 & 95.9 \\
%         \hline
%         DFR & \xmark/\cmark &  92.1 & 94.6\\
        
%         DFR+ExMap (ours) & \xmark/\xmark & 92.6 & 94.3
%         \\
%         \hline
%         JTT & \xmark/\cmark & 78.9 & 88.2 \\  
        
%         JTT+ExMap (ours) & \xmark/\xmark & 79.4 & 88.9\\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Worst group and mean accuracy on Waterbirds with two different clustering methods - kmeans and Spectral.}
%     \label{tab:ablate2}
% \end{table}

\begin{table}[!t]
    \centering
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcll}
        \toprule
        \textbf{Methods} & \textbf{Group Info} & \textbf{WGA(\%)} \color{Green}{$\uparrow$} & \textbf{Mean(\%)} \color{Green}{$\uparrow$} \\
        \midrule
        Base (ERM) & \xmark/\xmark & 41.1 & 95.9 \\
        \hline
        \rowcolor{gray!25}
        DFR & \xmark/\cmark &  92.1 & 96.7\\
        
        DFR+ExMap (ours) & \xmark/\xmark & 92.6 & 96.0
        \\
        \hline
        \rowcolor{gray!25}
        JTT & \xmark/\cmark & 86.7 & 93.3 \\  
        
        JTT+ExMap (ours) & \xmark/\xmark & 86.9 & 90.0\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}\caption{Worst group and mean accuracy on Waterbirds for two different retraining strategies - JTT and DFR.}\vspace{-5mm}
    \label{tab:ablate2}
\end{table}






==> ExMap-3/sec/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

The group robustness paradigm for deep learning classifiers raises important questions for when deep learning models succeed, but more importantly, \textit{when they fail}. However, most of current research focuses on the setting where group labels are available. This assumption is impractical for real-world scenarios, where the underlying spurious correlations in the data may not be known apriori. While recent work investigating unsupervised group robustness mechanisms have shown promise, we show that further improvements are possible. In our work, we propose ExMap, where we cluster explainable heatmaps to generate pseudo-labels for the validation data. These pseudo-labels are then used on off-the-shelf group robustness learning mechanisms in use today. In addition to showing why using heatmaps over raw features is useful in this setting, our results demonstrate the efficacy of this approach on a range of benchmark datasets, in both the single and multi-shortcut settings. We are able to further close the gap to supervised counterparts, and outperform partially supervised and unsupervised baselines. Finally, ExMap opens up interesting avenues to further leverage explainability heatmaps in group robust learning. 







